SEMOUR: A Scripted Emotional Speech Repository for Urdu

Designing reliable Speech Emotion Recognition systems is a complex task that inevitably requires sufficient data for training purposes. Such extensive datasets are currently available in only a few languages, including English, German, and Italian. In this paper, we present SEMOUR, the first scripted database of emotion-tagged speech in the Urdu language, to design an Urdu Speech Recognition System. Our gender-balanced dataset contains 15,040 unique instances recorded by eight professional actors eliciting a syntactically complex script. The dataset is phonetically balanced, and reliably exhibits a varied set of emotions as marked by the high agreement scores among human raters in experiments. We also provide various baseline speech emotion prediction scores on the database, which could be used for various applications like personalized robot assistants, diagnosis of psychological disorders, and getting feedback from a low-tech-enabled population, etc. On a random test sample, our model correctly predicts an emotion with a state-of-the-art 92% accuracy.

==> Supporting Libraries/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> references.tex <==
@inproceedings{robots,
author = {You, Yuhui and Fogelson, Mitchell and Cheng, Kelvin and Stenger, Bjorn},
title = {EMI: An Expressive Mobile Interactive Robot},
year = {2020},
isbn = {9781450368193},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3334480.3382852},
doi = {10.1145/3334480.3382852},
booktitle = {Extended Abstracts of the 2020 CHI Conference on Human Factors in Computing Systems},
pages = {1–8},
numpages = {8},
keywords = {robot design, emotional robot, robot tolerance, human-robot interaction},
location = {Honolulu, HI, USA},
series = {CHI EA '20}
}
@inproceedings{agents,
author = {Chin, Hyojin and Molefi, Lebogang Wame and Yi, Mun Yong},
title = {Empathy Is All You Need: How a Conversational Agent Should Respond to Verbal Abuse},
year = {2020},
isbn = {9781450367080},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3313831.3376461},
doi = {10.1145/3313831.3376461},
booktitle = {Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
pages = {1–13},
numpages = {13},
keywords = {verbal abuse, virtual assistant, agent abuse, smart speaker, intelligent personal assistant, conversational agent},
location = {Honolulu, HI, USA},
series = {CHI '20}
}

@inproceedings{weather,
author = {Scott, Kristen M. and Ashby, Simone and Hanna, Julian},
title = {"Human, All Too Human": NOAA Weather Radio and the Emotional Impact of Synthetic Voices},
year = {2020},
isbn = {9781450367080},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3313831.3376338},
doi = {10.1145/3313831.3376338},
booktitle = {Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
pages = {1–9},
numpages = {9},
keywords = {anthropomorphism, noaa weather radio, uncanny valley, text-to-speech, synthetic speech},
location = {Honolulu, HI, USA},
series = {CHI '20}
}

\cite{abuse}
@inproceedings{abuse,
author = {Vashistha, Aditya and Garg, Abhinav and Anderson, Richard and Raza, Agha Ali},
title = {Threats, Abuses, Flirting, and Blackmail: Gender Inequity in Social Media Voice Forums},
year = {2019},
isbn = {9781450359702},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3290605.3300302},
doi = {10.1145/3290605.3300302},
booktitle = {Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
pages = {1–13},
numpages = {13},
keywords = {social media, hci4d, ivr, voice forum, india, women, pakistan, gender},
location = {Glasgow, Scotland Uk},
series = {CHI '19}
}

@article{RUSSELL1977273,

title = "Evidence for a three-factor theory of emotions",

journal = "Journal of Research in Personality",

volume = "11",

number = "3",

pages = "273 - 294",

year = "1977",

issn = "0092-6566",

doi = "https://doi.org/10.1016/0092-6566(77)90037-X",

url = "http://www.sciencedirect.com/science/article/pii/009265667790037X",

author = "James A Russell and Albert Mehrabian"

}
@inproceedings{application_yoon2007study,
  title={A study of speech emotion recognition and its application to mobile services},
  author={Yoon, Won-Joong and Cho, Youn-Ho and Park, Kyu-Sik},
  booktitle={International Conference on Ubiquitous Intelligence and Computing},
  pages={758--766},
  year={2007},
  organization={Springer}
}
@inproceedings{application_deep2,
  title={Ordinal Learning for Emotion Recognition in Customer Service Calls},
  author={Han, Wenjing and Jiang, Tao and Li, Yan and Schuller, Bj{\"o}rn and Ruan, Huabin},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6494--6498},
  year={2020},

  address = {Barcelona, Spain},
  publisher = {IEEE}
}

@inproceedings{application_smarthome,
  title={The effect of emotional speech on a smart-home application},
  author={Kostoulas, Theodoros and Mporas, Iosif and Ganchev, Todor and Fakotakis, Nikos},
  booktitle={International Conference on Industrial, Engineering and Other Applications of Applied Intelligent Systems},
  pages={305--310},
  year={2008},
  organization={Springer},
  address = {Wroclaw, Poland},
  publisher = {Springer, Berlin, Heidelberg}
}

@InProceedings{application_elderly,
author="Castillo, Jos{\'e} Carlos
and Fern{\'a}ndez-Caballero, Antonio
and Castro-Gonz{\'a}lez, {\'A}lvaro
and Salichs, Miguel A.
and L{\'o}pez, Mar{\'i}a T.",
editor="Pecchia, Leandro
and Chen, Liming Luke
and Nugent, Chris
and Bravo, Jos{\'e}",
title="A Framework for Recognizing and Regulating Emotions in the Elderly",
booktitle="Ambient Assisted Living and Daily Activities",
year="2014",
publisher="Springer International Publishing",
address="Cham",
pages="320--327",
isbn="978-3-319-13105-4"
}

@inproceedings{urdufreqwords,
  title={Corpus based Urdu lexicon development},
  author={Ijaz, Madiha and Hussain, Sarmad},
  booktitle={the Proceedings of Conference on Language Technology (CLT07), University of Peshawar, Pakistan},
  volume={73},
  year={2007},
  address = {Pakistan},
  publisher = {Academia},
  pages = {12}
}
@misc{phonemelist,
  title={Speech assessment methods phonetic alphabet (SAMPA): Analysis of Urdu},
  author={Kabir, Hasan and Saleem, Abdul Mannan},
  journal={CRULP Annual Student Report published in Akhbar-e-Urdu},
  year={2002},
  pages = {6-11},
  numpages = {6}
}

@inproceedings{mcfee2015librosa,
  title={librosa: Audio and music signal analysis in python},
  author={McFee, Brian and Raffel, Colin and Liang, Dawen and Ellis, Daniel PW and McVicar, Matt and Battenberg, Eric and Nieto, Oriol},
  booktitle={Proceedings of the 14th python in science conference},
  volume={8},
  pages={18--25},
  year={2015},
  address = {Austin, Texas},
  publisher = {Academia}
}

@misc{eberhard2020ethnologue,
  title={Ethnologue: Languages of the world. 23rd edn. Dallas},
  organization={SIL International},
  author={Eberhard, David M and Simons, Gary F and Fennig, Charles D},
  journal={Online: https://www. ethnologue. com},
  year={2020},
  volume = {23}
}

@InProceedings{zia2018,
  author = {Haris Bin Zia ,Agha Ali Raza and Awais Athar},
  title = {PronouncUR: An Urdu Pronunciation Lexicon Generator},
  booktitle = {Proceedings of the Eleventh International Conference on Language Resources and Evaluation (LREC 2018)},
  year = {2018},
  month = {may},
  date = {7-12},
  location = {Miyazaki, Japan},
  publisher = {European Language Resources Association (ELRA)},
  address = {Paris, France},
  isbn = {979-10-95546-00-9},
  language = {english},
  numpages = {5}
  }
    
@inproceedings{regimtes,
  title={Building and analysing emotion corpus of the Arabic speech},
  author={Meddeb, Mohamed and Karray, Hichem and Alimi, Adel M},
  booktitle={2017 1st International Workshop on Arabic Script Analysis and Recognition (ASAR)},
  pages={134--139},
  year={2017},
  address = {Nancy, France},
  publisher = {IEEE},
  doi = {10.1109/ASAR.2017.8067775}
}

@article{shemo,
  title={ShEMO: a large-scale validated database for Persian speech emotion detection},
  author={Nezami, Omid Mohamad and Lou, Paria Jamshid and Karami, Mansoureh},
  journal={Language Resources and Evaluation},
  volume={53},
  number={1},
  pages={1--16},
  year={2019},
  publisher={Springer}
}
@inproceedings{urdu,
  title={Cross lingual speech emotion recognition: Urdu vs. western languages},
  author={Latif, Siddique and Qayyum, Adnan and Usman, Muhammad and Qadir, Junaid},
  booktitle={2018 International Conference on Frontiers of Information Technology (FIT)},
  pages={88--93},
  year={2018},
  address = {Islamabad, Pakistan, Pakistan},
  publisher = {IEEE},
  doi = {10.1109/FIT.2018.00023}
}
@article{tures,
  title={Recognizing emotion from Turkish speech using acoustic features},
  author={Oflazoglu, Caglar and Yildirim, Serdar},
  journal={EURASIP Journal on Audio, Speech, and Music Processing},
  volume={2013},
  number={1},
  pages={26},
  year={2013},
  publisher={Springer}
}
@article{baum1,
  title={BAUM-1: A spontaneous audio-visual face database of affective and mental states},
  author={Zhalehpour, Sara and Onder, Onur and Akhtar, Zahid and Erdem, Cigdem Eroglu},
  journal={IEEE Transactions on Affective Computing},
  volume={8},
  number={3},
  pages={300--313},
  year={2016},
  publisher={IEEE}
}
@inproceedings{recola,
  title={Introducing the RECOLA multimodal corpus of remote collaborative and affective interactions},
  author={Ringeval, Fabien and Sonderegger, Andreas and Sauer, Juergen and Lalanne, Denis},
  booktitle={2013 10th IEEE international conference and workshops on automatic face and gesture recognition (FG)},
  pages={1--8},
  year={2013},
  address = {Shanghai, China},
  publisher = {IEEE},
  doi={10.1109/FG.2013.6553805}
}
@inproceedings{casia,
  title={Design of speech corpus for mandarin text to speech},
  author={Zhang, Jianhua Tao Fangzhou Liu Meng and Jia, Huibin},
  booktitle={The Blizzard Challenge 2008 workshop},
  year={2008},
  pages={4},
  address = {Brisbane, Australia},
  publisher = {International Speech Communication Association}
}

@inproceedings{cass,
  title={CASS: A phonetically transcribed corpus of Mandarin spontaneous speech},
  author={Li, Aijun and Zheng, Fang and Byrne, William and Fung, Pascale and Kamm, Terri and Liu, Yi and Song, Zhanjiang and Ruhi, Umar and Venkataramani, Veera and Chen, Xiaoxia},
  booktitle={Sixth International Conference on Spoken Language Processing},
  year={2000},
  pages={485-488},
  address = {Beijing, China},
  publisher = {International Speech Communication Association}
}
@article{cheavd,
  title={CHEAVD: a Chinese natural emotional audio--visual database},
  author={Li, Ya and Tao, Jianhua and Chao, Linlin and Bao, Wei and Liu, Yazhu},
  journal={Journal of Ambient Intelligence and Humanized Computing},
  volume={8},
  number={6},
  pages={913--924},
  year={2017},
  publisher={Springer}
}

@inproceedings{keioesd,
  title={Emotional speech synthesis using subspace constraints in prosody},
  author={Mori, Shinya and Moriyama, Tsuyoshi and Ozawa, Shinji},
  booktitle={2006 IEEE International Conference on Multimedia and Expo},
  pages={1093--1096},
  year={2006},
  address = {Toronto, Ont., Canada},
  publisher = {IEEE},
  doi = {10.1109/ICME.2006.262725}
}

@inproceedings{emovo,
  title={EMOVO corpus: an Italian emotional speech database},
  author={Costantini, Giovanni and Iaderola, Iacopo and Paoloni, Andrea and Todisco, Massimiliano},
  booktitle={International Conference on Language Resources and Evaluation (LREC 2014)},
  pages={3501--3504},
  year={2014},
  organization={European Language Resources Association (ELRA)},
  address = {Reykjavik, Iceland},
  publisher = {European Language Resources Association}
}
@inproceedings{emodb,
  title={A database of German emotional speech},
  author={Burkhardt, Felix and Paeschke, Astrid and Rolfes, Miriam and Sendlmeier, Walter F and Weiss, Benjamin},
  booktitle={Ninth European Conference on Speech Communication and Technology},
  year={2005},
  numpages = {4},
  pages = {1517-1520},
  address = {Lisbon, Portugal},
  publisher = {International Speech Communication Association}
}
@inproceedings{vam,
  title={The Vera am Mittag German audio-visual emotional speech database},
  author={Grimm, Michael and Kroschel, Kristian and Narayanan, Shrikanth},
  booktitle={2008 IEEE international conference on multimedia and expo},
  pages={865--868},
  year={2008},
  address = {Hannover, Germany},
  publisher = {IEEE}
}
@inproceedings{faubaibo,
  title={Releasing a thoroughly annotated and processed spontaneous emotional database: the FAU Aibo Emotion Corpus},
  author={Batliner, Anton and Steidl, Stefan and N{\"o}th, Elmar},
  booktitle={Proc. of a Satellite Workshop of LREC},
  pages={28},
  year={2008},
  address = {Marrakesh, Morocco},
  publisher = {European Language Resources Association}
}
@article{iemocap,
  title={IEMOCAP: Interactive emotional dyadic motion capture database},
  author={Busso, Carlos and Bulut, Murtaza and Lee, Chi-Chun and Kazemzadeh, Abe and Mower, Emily and Kim, Samuel and Chang, Jeannette N and Lee, Sungbok and Narayanan, Shrikanth S},
  journal={Language resources and evaluation},
  volume={42},
  number={4},
  pages={335},
  year={2008},
  publisher={Springer}
}
@misc{savee,
  title={Surrey audio-visual expressed emotion (savee) database},
  author={Jackson, P and Haq, S},
  journal={University of Surrey: Guildford, UK},
  year={2014}
}
@article{ravsdess,
  title={The Ryerson Audio-Visual Database of Emotional Speech and Song (RAVDESS): A dynamic, multimodal set of facial and vocal expressions in North American English},
  author={Livingstone, Steven R and Russo, Frank A},
  journal={PloS one},
  volume={13},
  number={5},
  pages={e0196391},
  year={2018},
  publisher={Public Library of Science San Francisco, CA USA}
}
@article{mspimprov,
  title={MSP-IMPROV: An acted corpus of dyadic interactions to study emotion perception},
  author={Busso, Carlos and Parthasarathy, Srinivas and Burmania, Alec and AbdelWahab, Mohammed and Sadoughi, Najmeh and Provost, Emily Mower},
  journal={IEEE Transactions on Affective Computing},
  volume={8},
  number={1},
  pages={67--80},
  year={2016},
  publisher={IEEE}
}
@inproceedings{vesus,
  title={VESUS: A Crowd-Annotated Database to Study Emotion Production and Perception in Spoken English.},
  author={Sager, Jacob and Shankar, Ravi and Reinhold, Jacob and Venkataraman, Archana},
  booktitle={INTERSPEECH},
  pages={316--320},
  year={2019},
  address = {Graz, Austria},
  publisher = {International Speech Communication Association}
}

@article{swain2018databases,
  title={Databases, features and classifiers for speech emotion recognition: a review},
  author={Swain, Monorama and Routray, Aurobinda and Kabisatpathy, Prithviraj},
  journal={International Journal of Speech Technology},
  volume={21},
  number={1},
  pages={93--120},
  year={2018},
  publisher={Springer}
}

@article{fayek2017evaluating,
  title={Evaluating deep learning architectures for Speech Emotion Recognition},
  author={Fayek, Haytham M and Lech, Margaret and Cavedon, Lawrence},
  journal={Neural Networks},
  volume={92},
  pages={60--68},
  year={2017},
  publisher={Elsevier}
}

@article{chen20183,
  title={3-D convolutional recurrent neural networks with attention model for speech emotion recognition},
  author={Chen, Mingyi and He, Xuanji and Yang, Jing and Zhang, Han},
  journal={IEEE Signal Processing Letters},
  volume={25},
  number={10},
  pages={1440--1444},
  year={2018},
  publisher={IEEE}
}

@article{zhao2019speech,
  title={Speech emotion recognition using deep 1D \& 2D CNN LSTM networks},
  author={Zhao, Jianfeng and Mao, Xia and Chen, Lijiang},
  journal={Biomedical Signal Processing and Control},
  volume={47},
  pages={312--323},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{li2019attentive,
  title={Attentive to Individual: A Multimodal Emotion Recognition Network with Personalized Attention Profile.},
  author={Li, Jeng-Lin and Lee, Chi-Chun},
  booktitle={INTERSPEECH},
  pages={211--215},
  year={2019},
  address = {Graz, Austria},
  publisher = {International Speech Communication Association}
}

@article{sahidullah2012design,
  title={Design, analysis and experimental evaluation of block based transformation in MFCC computation for speaker recognition},
  author={Sahidullah, Md and Saha, Goutam},
  journal={Speech communication},
  volume={54},
  number={4},
  pages={543--565},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{schuller2016interspeech,
  title={The interspeech 2016 computational paralinguistics challenge: Deception, sincerity \& native language},
  author={Schuller, Bj{\"o}rn and Steidl, Stefan and Batliner, Anton and Hirschberg, Julia and Burgoon, Judee K and Baird, Alice and Elkins, Aaron and Zhang, Yue and Coutinho, Eduardo and Evanini, Keelan and others},
  booktitle={17TH ANNUAL CONFERENCE OF THE INTERNATIONAL SPEECH COMMUNICATION ASSOCIATION (INTERSPEECH 2016), VOLS 1-5},
  pages={2001--2005},
  year={2016},
  address = {San Francisco, CA, USA},
  publisher = {International Speech Communication Association}
}

@article{eyben2015geneva,
  title={The Geneva minimalistic acoustic parameter set (GeMAPS) for voice research and affective computing},
  author={Eyben, Florian and Scherer, Klaus R and Schuller, Bj{\"o}rn W and Sundberg, Johan and Andr{\'e}, Elisabeth and Busso, Carlos and Devillers, Laurence Y and Epps, Julien and Laukka, Petri and Narayanan, Shrikanth S and others},
  journal={IEEE transactions on affective computing},
  volume={7},
  number={2},
  pages={190--202},
  year={2015},
  publisher={IEEE}
}

@inproceedings{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  booktitle={3rd International Conference on Learning Representations, ICLR 2015},
  year={2015},
  numpages = 15,
  publisher={Computational and Biological Learning Society},
  address={San Diego, CA, USA}
}


@inproceedings{parry2019analysis,
  title={Analysis of Deep Learning Architectures for Cross-Corpus Speech Emotion Recognition.},
  author={Parry, Jack and Palaz, Dimitri and Clarke, Georgia and Lecomte, Pauline and Mead, Rebecca and Berger, Michael and Hofer, Gregor},
  booktitle={INTERSPEECH},
  pages={1656--1660},
  year={2019},
  address = {Graz, Austria},
  publisher = {International Speech Communication Association}
}

@inproceedings{sebastian2019fusion,
  title={Fusion Techniques for Utterance-Level Emotion Recognition Combining Speech and Transcripts.},
  author={Sebastian, Jilt and Pierucci, Piero},
  booktitle={INTERSPEECH},
  pages={51--55},
  year={2019},
  address = {Graz, Austria},
  publisher = {International Speech Communication Association}
}

@inproceedings{xu2019autonomous,
  title={Autonomous Emotion Learning in Speech: A View of Zero-Shot Speech Emotion Recognition.},
  author={Xu, Xinzhou and Deng, Jun and Cummins, Nicholas and Zhang, Zixing and Zhao, Li and Schuller, Bj{\"o}rn W},
  booktitle={INTERSPEECH},
  pages={949--953},
  year={2019},
  address = {Graz, Austria},
  publisher = {International Speech Communication Association}
}

@inproceedings{chatziagapi2019data,
  title={Data Augmentation Using GANs for Speech Emotion Recognition.},
  author={Chatziagapi, Aggelina and Paraskevopoulos, Georgios and Sgouropoulos, Dimitris and Pantazopoulos, Georgios and Nikandrou, Malvina and Giannakopoulos, Theodoros and Katsamanis, Athanasios and Potamianos, Alexandros and Narayanan, Shrikanth},
  booktitle={INTERSPEECH},
  pages={171--175},
  year={2019},
  publisher = {International Speech Communication Association},
  address = {Graz, Austria}
}

@article{stevens1937scale,
  title={A scale for the measurement of the psychological magnitude pitch},
  author={Stevens, Stanley Smith and Volkmann, John and Newman, Edwin B},
  journal={The Journal of the Acoustical Society of America},
  volume={8},
  number={3},
  pages={185--190},
  year={1937},
  publisher={Acoustical Society of America}
}

@article{ekman,
  title={An argument for basic emotions},
  author={Ekman, Paul},
  journal={Cognition \& emotion},
  volume={6},
  number={3-4},
  pages={169--200},
  year={1992},
  publisher={Taylor \& Francis}
}



@article{sajjad2020clustering,
  title={Clustering-Based Speech Emotion Recognition by Incorporating Learned Features and Deep BiLSTM},
  author={Sajjad, Muhammad and Kwon, Soonil and others},
  journal={IEEE Access},
  volume={8},
  pages={79861--79875},
  year={2020},
  publisher={IEEE}
}
@inproceedings{raza2009design,
  title={Design and development of phonetically rich Urdu speech corpus},
  author={Raza, Agha Ali and Hussain, Sarmad and Sarfraz, Huda and Ullah, Inam and Sarfraz, Zahid},
  booktitle={2009 oriental COCOSDA international conference on speech database and assessments},
  pages={38--43},
  year={2009},
  publisher = {IEEE},
  address = {Urumqi, China}
}



@article{wu2011automatic,
  title={Automatic speech emotion recognition using modulation spectral features},
  author={Wu, Siqing and Falk, Tiago H and Chan, Wai-Yip},
  journal={Speech communication},
  volume={53},
  number={5},
  pages={768--785},
  year={2011},
  publisher={Elsevier}
}

@INPROCEEDINGS{accents,
  author={M. {Qasim} and S. {Nawaz} and S. {Hussain} and T. {Habib}},
  booktitle={2016 Conference of The Oriental Chapter of International Committee for Coordination and Standardization of Speech Databases and Assessment Techniques (O-COCOSDA)}, 
  title={Urdu speech recognition system for district names of Pakistan: Development, challenges and solutions}, 
  year={2016},
  volume={},
  number={},
  pages={28-32},
  doi={10.1109/ICSDA.2016.7918979},
  address = {Bali, Indonesia},
  publisher = {IEEE}
  }
  
  @INPROCEEDINGS{dialects,
  author={S. M. {Ghulam} and T. R. {Soomro}},
  booktitle={2018 International Conference on Computing, Mathematics and Engineering Technologies (iCoMET)}, 
  title={Twitter and Urdu}, 
  year={2018},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICOMET.2018.8346370},
  address = {Sukkur, Pakistan},
  publisher = {IEEE}
  
  }
  
  @INPROCEEDINGS{ali2012medium,
  title={A medium vocabulary Urdu isolated words balanced corpus for automatic speech recognition},
  author={Ali, Hazrat and Ahmad, Nasir and Yahya, Khawaja M and Farooq, Omar},
  booktitle={2012 international conference on electronics computer technology (ICECT 2012)},
  pages={473--476},
  publisher={IEEE},
  address = {Kanyakumari, India},
  year={2012}
}


@article{williams1972emotions,
  title={Emotions and speech: Some acoustical correlates},
  author={Williams, Carl E and Stevens, Kenneth N},
  journal={The Journal of the Acoustical Society of America},
  volume={52},
  number={4B},
  pages={1238--1250},
  year={1972},
  publisher={Acoustical Society of America}
}

@inproceedings{engberg1997design,
  title={Design, recording and verification of a Danish emotional speech database},
  author={Engberg, Inger S and Hansen, Anya Varnich and Andersen, Ove and Dalsgaard, Paul},
  booktitle={Fifth European conference on speech communication and technology},
  year={1997}
}

@article{douglas2003emotional,
  title={Emotional speech: Towards a new generation of databases},
  author={Douglas-Cowie, Ellen and Campbell, Nick and Cowie, Roddy and Roach, Peter},
  journal={Speech communication},
  volume={40},
  number={1-2},
  pages={33--60},
  year={2003},
  publisher={Elsevier}
}

@article{jurgens2015effect,
  title={Effect of acting experience on emotion expression and recognition in voice: Non-actors provide better stimuli than expected},
  author={J{\"u}rgens, Rebecca and Grass, Annika and Drolet, Matthis and Fischer, Julia},
  journal={Journal of nonverbal behavior},
  volume={39},
  number={3},
  pages={195--214},
  year={2015},
  publisher={Springer}
}


@article{livingstone2018ryerson,
  title={The Ryerson Audio-Visual Database of Emotional Speech and Song (RAVDESS): A dynamic, multimodal set of facial and vocal expressions in North American English},
  author={Livingstone, Steven R and Russo, Frank A},
  journal={PloS one},
  volume={13},
  number={5},
  pages={e0196391},
  year={2018},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{belin2008montreal,
  title={The Montreal Affective Voices: a validated set of nonverbal affect bursts for research on auditory affective processing},
  author={Belin, Pascal and Fillion-Bilodeau, Sarah and Gosselin, Fr{\'e}d{\'e}ric},
  journal={Behavior research methods},
  volume={40},
  number={2},
  pages={531--539},
  year={2008},
  publisher={Springer}
}

@article{banziger2012introducing,
  title={Introducing the Geneva multimodal expression corpus for experimental research on emotion perception.},
  author={B{\"a}nziger, Tanja and Mortillaro, Marcello and Scherer, Klaus R},
  journal={Emotion},
  volume={12},
  number={5},
  pages={1161},
  year={2012},
  publisher={American Psychological Association}
}

@article{castro2010recognizing,
  title={Recognizing emotions in spoken language: A validated set of Portuguese sentences and pseudosentences for research on emotional prosody},
  author={Castro, S{\~a}o Lu{\'\i}s and Lima, C{\'e}sar F},
  journal={Behavior Research Methods},
  volume={42},
  number={1},
  pages={74--81},
  year={2010},
  publisher={Springer}
}

@article{ekman1969pan,
  title={Pan-cultural elements in facial displays of emotion},
  author={Ekman, Paul and Sorenson, E Richard and Friesen, Wallace V},
  journal={Science},
  volume={164},
  number={3875},
  pages={86--88},
  year={1969},
  publisher={American Association for the Advancement of Science}
}

@article{izard1992basic,
  title={Basic emotions, relations among emotions, and emotion-cognition relations.},
  author={Izard, Carroll E},
  year={1992},
  publisher={American Psychological Association}
}

@book{tomkins1962affect,
  title={Affect imagery consciousness: Volume I: The positive affects},
  author={Tomkins, Silvan S},
  volume={1},
  year={1962},
  publisher={Springer}
}

@article{ekman1992argument,
  title={An argument for basic emotions},
  author={Ekman, Paul},
  journal={Cognition \& emotion},
  volume={6},
  number={3-4},
  pages={169--200},
  year={1992},
  publisher={Taylor \& Francis}
}

@article{russell1994there,
  title={Is there universal recognition of emotion from facial expression? A review of the cross-cultural studies.},
  author={Russell, James A},
  journal={Psychological bulletin},
  volume={115},
  number={1},
  pages={102},
  year={1994},
  publisher={American Psychological Association}
}

@article{ortony1990s,
  title={What's basic about basic emotions?},
  author={Ortony, Andrew and Turner, Terence J},
  journal={Psychological review},
  volume={97},
  number={3},
  pages={315},
  year={1990},
  publisher={American Psychological Association}
}


@article{schroder2003experimental,
  title={Experimental study of affect bursts},
  author={Schr{\"o}der, Marc},
  journal={Speech communication},
  volume={40},
  number={1-2},
  pages={99--116},
  year={2003},
  publisher={Elsevier}
}

@inproceedings{tato2002emotional,
  title={Emotional space improves emotion recognition},
  author={Tato, Raquel and Santos, Rocio and Kompe, Ralf and Pardo, Jos{\'e} M},
  booktitle={Seventh International Conference on Spoken Language Processing},
  year={2002}
}

@inproceedings{batliner2004you,
  title={" You Stupid Tin Box"-Children Interacting with the AIBO Robot: A Cross-linguistic Emotional Speech Corpus.},
  author={Batliner, Anton and Hacker, Christian and Steidl, Stefan and N{\"o}th, Elmar and D'Arcy, Shona and Russell, Martin J and Wong, Michael},
  booktitle={International Conference on Language Resources and Evaluation (LREC 2004)},
  year={2004},
  address = {Lisbon, Portugal},
  publisher = {European Language Resources Association}
}


@inproceedings{cichosz2005low,
  title={Low-dimensional feature space derivation for emotion recognition},
  author={Cichosz, Jaroslaw and Slot, Krzysztof},
  booktitle={Ninth European conference on speech communication and technology},
  year={2005}
}

@inproceedings{pao2005combining,
  title={Combining acoustic features for improved emotion recognition in mandarin speech},
  author={Pao, Tsang-Long and Chen, Yu-Te and Yeh, Jun-Heng and Liao, Wen-Yuan},
  booktitle={International conference on affective computing and intelligent interaction},
  pages={279--285},
  year={2005},
  organization={Springer}
}

@article{harimi2014database,
  title={A database for automatic Persian speech emotion recognition: collection, processing and evaluation},
  author={Harimi, Ali and Esmaileyan, Zeynab},
  journal={International Journal of Engineering},
  volume={27},
  number={1},
  pages={79--90},
  year={2014},
  publisher={Materials and Energy Research Center}
}

@book{buck1988human,
  title={Human motivation and emotion},
  author={Buck, Ross},
  year={1988},
  publisher={John Wiley \& Sons}
}

@article{ross2007epistemological,
  title={Epistemological models and culture conflict: Menominee and euro-american hunters in wisconsin},
  author={Ross, Norbert and Medin, Doug and Cox, Doug},
  journal={Ethos},
  volume={35},
  number={4},
  pages={478--515},
  year={2007},
  publisher={Wiley Online Library}
}

@phdthesis{fernandez2004computational,
  title={A computational model for the automatic recognition of affect in speech},
  author={Fernandez, Raul},
  year={2004},
  school={Massachusetts Institute of Technology}
}

@article{russell1999core,
  title={Core affect, prototypical emotional episodes, and other things called emotion: dissecting the elephant.},
  author={Russell, James A and Barrett, Lisa Feldman},
  journal={Journal of personality and social psychology},
  volume={76},
  number={5},
  pages={805},
  year={1999},
  publisher={American Psychological Association}
}

@inproceedings{burkhardt2005database,
  title={A database of German emotional speech},
  author={Burkhardt, Felix and Paeschke, Astrid and Rolfes, Miriam and Sendlmeier, Walter F and Weiss, Benjamin},
  booktitle={Ninth European Conference on Speech Communication and Technology},
  year={2005}
}

@article{ekman1976pictures,
  title={Pictures of facial affect},
  author={Ekman, Paul},
  journal={Consulting Psychologists Press},
  year={1976},
  publisher={Palo Alto}
}

@article{mazurski1993new,
  title={A new series of slides depicting facial expressions of affect: A comparison with the pictures of facial affect series},
  author={Mazurski, Evalynn J and Bond, Nigel W},
  journal={Australian Journal of Psychology},
  volume={45},
  number={1},
  pages={41--47},
  year={1993},
  publisher={Wiley Online Library}
}

@article{wang1999development,
  title={The development of a series of photographs of Chinese facial expressions of emotion},
  author={Wang, Lei and Markham, Roslyn},
  journal={Journal of Cross-Cultural Psychology},
  volume={30},
  number={4},
  pages={397--410},
  year={1999},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@inproceedings{kanade2000comprehensive,
  title={Comprehensive database for facial expression analysis},
  author={Kanade, Takeo and Cohn, Jeffrey F and Tian, Yingli},
  booktitle={Proceedings Fourth IEEE International Conference on Automatic Face and Gesture Recognition (Cat. No. PR00580)},
  pages={46--53},
  year={2000},
  publisher={IEEE}
}


@article{el2011survey,
  title={Survey on speech emotion recognition: Features, classification schemes, and databases},
  author={El Ayadi, Moataz and Kamel, Mohamed S and Karray, Fakhri},
  journal={Pattern Recognition},
  volume={44},
  number={3},
  pages={572--587},
  year={2011},
  publisher={Elsevier}
}

@article{gomez2007relationships,
  title={Relationships between musical structure and psychophysiological measures of emotion.},
  author={Gomez, Patrick and Danuser, Brigitta},
  journal={Emotion},
  volume={7},
  number={2},
  pages={377},
  year={2007},
  publisher={American Psychological Association}
}

@book{schubert1999measurement,
  title={Measurement and time series analysis of emotion in music},
  author={Schubert, Emery},
  volume={1},
  year={1999},
  publisher={University of New South Wales Sydney}
}

@inproceedings{schuller2004speech,
  title={Speech emotion recognition combining acoustic features and linguistic information in a hybrid support vector machine-belief network architecture},
  author={Schuller, Bj{\"o}rn and Rigoll, Gerhard and Lang, Manfred},
  booktitle={2004 IEEE International Conference on Acoustics, Speech, and Signal Processing},
  volume={1},
  pages={I--577},
  year={2004},
  Publisher={IEEE}
}

@article{france2000acoustical,
  title={Acoustical properties of speech as indicators of depression and suicidal risk},
  author={France, Daniel Joseph and Shiavi, Richard G and Silverman, Stephen and Silverman, Marilyn and Wilkes, M},
  journal={IEEE transactions on Biomedical Engineering},
  volume={47},
  number={7},
  pages={829--837},
  year={2000},
  publisher={IEEE}
}


@inproceedings{sager2019vesus,
  title={VESUS: A Crowd-Annotated Database to Study Emotion Production and Perception in Spoken English.},
  author={Sager, Jacob and Shankar, Ravi and Reinhold, Jacob and Venkataraman, Archana},
  booktitle={INTERSPEECH},
  publisher={International Speech Communication Association},
  pages={316--320},
  year={2019}
}


@inproceedings{douglas2005multimodal,
  title={Multimodal databases of everyday emotion: Facing up to complexity},
  author={Douglas-Cowie, Ellen and Devillers, Laurence and Martin, Jean-Claude and Cowie, Roddy and Savvidou, Suzie and Abrilian, Sarkis and Cox, Cate},
  booktitle={Ninth European conference on speech communication and technology},
  year={2005},
  pages = {4},
  address = {Lisbon, Portugal},
  publisher = {International Speech Communication Association}
}

@inproceedings{cauldwell2000did,
  title={Where did the anger go? The role of context in interpreting emotion in speech},
  author={Cauldwell, Richard T},
  booktitle={ISCA Tutorial and Research Workshop (ITRW) on Speech and Emotion},
  year={2000},
  numpages = {5},
  address = {Newcastle, Northern Ireland, UK},
  publisher = {International Speech Communication Association}
}

@inproceedings{batliner2000desperately,
  title={Desperately seeking emotions or: Actors, wizards, and human beings},
  author={Batliner, Anton and Fischer, Kerstin and Huber, Richard and Spilker, J{\"o}rg and N{\"o}th, Elmar},
  booktitle={ISCA tutorial and research workshop (ITRW) on speech and emotion},
  year={2000},
  address = {Newcastle, Northern Ireland, UK},
  publisher = {International Speech Communication Association},
  numpages = 6
}

@article{scherer2003vocal,
  title={Vocal communication of emotion: A review of research paradigms},
  author={Scherer, Klaus R},
  journal={Speech communication},
  volume={40},
  number={1-2},
  pages={227--256},
  year={2003},
  publisher={Elsevier}
}
@article{devillers2005challenges,
  title={Challenges in real-life emotion annotation and machine learning based detection},
  author={Devillers, Laurence and Vidrascu, Laurence and Lamel, Lori},
  journal={Neural Networks},
  volume={18},
  number={4},
  pages={407--422},
  year={2005},
  publisher={Elsevier}
}
